Co-design Hardware and Algorithm for Vector Search

Vector search has emerged as the foundation for large-scale information retrieval and machine learning systems, with search engines like Google and Bing processing tens of thousands of queries per second on petabyte-scale document datasets by evaluating vector similarities between encoded query texts and web documents. As performance demands for vector search systems surge, accelerated hardware offers a promising solution in the post-Moore's Law era. We introduce \textit{FANNS}, an end-to-end and scalable vector search framework on FPGAs. Given a user-provided recall requirement on a dataset and a hardware resource budget, \textit{FANNS} automatically co-designs hardware and algorithm, subsequently generating the corresponding accelerator. The framework also supports scale-out by incorporating a hardware TCP/IP stack in the accelerator. \textit{FANNS} attains up to 23.0$\times$ and 37.2$\times$ speedup compared to FPGA and CPU baselines, respectively, and demonstrates superior scalability to GPUs, achieving 5.5$\times$ and 7.6$\times$ speedup in median and 95\textsuperscript{th} percentile (P95) latency within an eight-accelerator configuration. The remarkable performance of \textit{FANNS} lays a robust groundwork for future FPGA integration in data centers and AI supercomputers.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\ul{\textit{FANNS} Scalability.} 
\textit{FANNS} assumes that the dataset is stored in the device memory instead of the host CPU memory, because the throughput of PCIe can be a significant limitation for performance.
In fact, not only \textit{FANNS} but many other hardware-accelerated data management tasks make such assumptions. 
For example, \citet{shanbhag2020study} shows that in-GPU-memory database is significantly faster than the case of transferring data to GPUs on demand.
Faiss also stores data in GPU memory to achieve high ANNS performance. 
One concern about this assumption is that accelerators typically have much smaller memory capacity than the host server. We hereby analyze the \textit{FANNS} scalability. 
The largest vector datasets publically available contain one billion vectors~\cite{simhadri2022results}. 
 It requires around 20 GB of memory for the entire dataset by quantizing the vectors to 16-byte PQ codes and storing the vector IDs using 4-byte integers.
Thus, we need three U280 FPGAs (8 GB memory) or two U55c FPGAs (16 GB memory) running in parallel. 
Apart from the off-the-shelf FPGA models, the research community has been building powerful FPGAs. 
Enzian~\cite{cock2022enzian}, for example, equips the FPGA with 512 GB of memory, more than enough to hold billion-scale vector datasets on a single machine.


% This is not a surprise given the results of existing research on FPGA and GPU accelerated databases and related applications~\cite{}, while the performance of the operator-offloading model can be significantly restricted by the PCIe bandwidth~\cite{}. 

\ul{FPGAs versus GPUs.} 
Though achieving better ANNS efficiency than GPU (normalizing the performance by theoretical computation capability), FPGAs still have a performance gap compared to GPUs. 
This is not a big surprise because GPUs have two orders of magnitude higher computation capability than FPGAs. 
Due to this capability gap, GPUs typically outperform FPGA in workloads such as machine learning~\cite{nurvitadhi2017can}, relational database~\cite{he2008relational, halstead2013accelerating}, etc.
However, it is still worth studying FPGA-accelerated data management for several reasons.
First, FPGAs are becoming increasingly available in data centers. 
Most of the Microsoft Azure servers are already equipped with FPGAs. 
In the future, the integrated CPU-FPGA on the same chip~\cite{kegel2020method} will further extend the availability of reconfigurable hardware. 
Second, FPGA performance is evolving rapidly: the upcoming Versal FPGA (available in 2022) provides an order of magnitude better flop/s compared to the U280 (available in 2020), because Versal integrates the reconfigurable circuit with dedicated SIMD cores. 
Third, there are many forms of FPGA deployments beyond PCIe-based accelerators. 
For example, the network interface enables FPGAs to function as an independent service without involving the host server~\cite{100gbps};
some FPGAs contain cache-coherent links to CPUs~\cite{cock2022enzian}, allowing the two processors to work on the same workload seamlessly;
FPGAs can sit between CPU and memory/storage for near-data processing.
% embedded systems, computation at the edge, streaming architectures, smart-NICs, near storage or near memory processing, etc.
Finally, FPGAs shine on irregular parallelism and custom data types, thus they can outperform GPUs on such workloads~\cite{umuroglu2017finn}. 

% First, FPGAs have shown great energy efficiency because of their fully customizable circuits~\cite{qasaimeh2019comparing, betkaoui2010comparing, umuroglu2017finn}. 
% Second, FPGAs are increasingly available in data centers and in the cloud~\cite{caulfield2016cloud, aqua}. %  MS, AWS, Alibaba, 
% Third, FPGAs can be integrated with CPU on the same chip in the future according, making the reconfigurable hardware even more viable~\cite{kegel2020method}. %
% As a result, big companies such as Microsoft, Amazon, Alibaba, and Baidu have adopted FPGAs for various workloads including machine learning inference, database acceleration, network offloading, and security operations~\cite{caulfield2016cloud, aqua, chen2022fidas, firestone2018azure}.
% Due to the increasing popularity and the great potential of FPGAs, we study FPGA-based ANNS acceleration in this paper.


% The first one is, in the future FPGA can be fused with CPU in the same chip, and FPGA can work on part of the stuff. The energy consumption is good compare to GPUs. 
% The second one is that FPGA can also appear as a standlone service given the network port, serving as low-latency accelerator. 

==> fpga.tex <==
\section{Field Programmable Gate Arrays}
\label{sec:FPGA}
% What to include:

% * FPGA basics (compare with GPU? say much lower computation power, mainly for latency critical jobs?)

% * the target FPGA (HBM)

% * the high design cost

% * preliminaries: resource and clock


\textit{Hardware.} Field programmable gate array (FPGA) lies between general-purpose processors (e.g., CPUs) and application-speciﬁc integrated circuits (ASICs): it behaves like ASICs, yet its circuit can be reconfigured virtually infinite number of times, thus leveraging performance and design flexibility.
Developers can design arbitrary micro-architectures given the traits of specific applications, compile the design to a bitstream file representing the circuit configuration, and load the bitstream on FPGAs to start accelerating the applications. 
This is achieved by the hardware compiler which can map a logical design to the physical hardware units on FPGAs. These units mainly include (a) Block-RAM (BRAM) and the Xilinx-specific Ultra-RAM (URAM) as small yet fast on-chip memory, (b) Flip-Flops (FF) as registers, (c) Digital Signal Processors (DSP) as computing units, and (d) lookup-tables (LUT) as either memory or computing units. 


\textit{Programming Model.} Developing FPGA accelerators typically requires much more efforts compared with software designs. Traditionally, FPGAs are programmed by hardware description languages (HDL), such as Verilog and VHDL. Developers need to define the behavior of the circuit at the granularity of a single clock cycle. Recently, High-Level Synthesis (HLS) has become popular in the FPGA community. It allows programmers to develop the circuit at a higher level using C/C++ or OpenCL~\cite{vivado_hls, intel_opencl_fpga}. However, developing accelerators by HLS requires extra efforts to learn the specific hardware-friendly coding style and to fine-tune the performance by exploring a wide range of \textit{pragmas}. 

\textit{Target FPGA Device.} 
% Figure~\ref{fig:HBM-AXI} shows our target FPGA, Xilinx Alveo U280~\cite{xilinx_u280}, which is installed on a CPU-server as a plug-in accelerator. 
We target Alveo U280 FPGAs~\cite{xilinx_u280}, Xilinx's flagship FPGA for data center applications.
The card is installed on CPU server's PCIe slot.
Each card equips 8 GB High-Bandwidth Memory (HBM) that offers improved concurrency and bandwidth (up to 425 GB/s) compared to conventional DRAM~\cite{jun2017hbm, o2014highlights, wang2020shuhai}. 
The HBM contains 32 independent memory channels (banks) that can be accessed concurrently. 
% Thus, PQ codebooks can be distributed to these banks so that each bank only contains one or a few tables, and up to 32 tables can be looked up concurrently.

% \begin{figure}%[t]
% 	% full width, can be adjusted
%   \centering
%   \includegraphics[width=0.95\linewidth]{fig/HBM-AXI.png}
%   \vspace{-0.7em}
%   \caption{The Xilinx U280 FPGA board can serve as a plug-in accelerator over PCIe on a CPU server. The user-designed circuit kernel can access the high-bandwidth memory (8 GBs in total; 32 independent banks) through AXI interface.}
% %   \vspace*{-3mm}
%   \label{fig:HBM-AXI}
% \end{figure}


% \textit{Design Cost.} Developing FPGA accelerators typically requires much more efforts compared with software designs. Traditionally, FPGAs are programmed by hardware description languages (HDL), such as Verilog and VHDL. Developers need to define the behavior of the circuit at the granularity of a single clock cycle. Recently, High-Level Synthesis (HLS) has become popular in the FPGA community. It allows programmers to develop the circuit at a higher level using C/C++ or OpenCL~\cite{vivado_hls, intel_opencl_fpga}. However, developing accelerators by HLS requires extra efforts to learn the specific hardware-friendly coding style and to fine-tune the performance by exploring a wide range of \textit{pragmas}. Besides, unlike software projects that only need to target x86 and/or ARM, many FPGA projects are specific to certain FPGA models. \textit{As a result, the development cost of FPGA accelerators must be keep in mind when launching a project, and it is typically impossible to explore as many designs as software projects.}


% \subsection{Typical FPGA design: PE and dataflow}

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}


% (1) FPGAs are increasingly available
% (2) FPGAs are energy efficient
% (3) (novel architecture) FPGAs have the potential being integrated into CPU

Due to the end of Moore's law and Dennard Scaling, it is timely to study accelerator designs for emerging applications such as ANNS. 
%customized accelerators have been increasingly important to make data center applications efficient. 
GPUs, as the most popular accelerators in data centers, have already shown success in ANNS~\cite{johnson2019billion, wieschollek2016efficient, chen2019robustiq, chen2019vector} thanks to its incomparable computation capability and memory bandwidth.
Though not as powerful as GPUs in terms of peak performance, FPGAs have also gained increasing attention by many companies for three reasons. 
% FFT: Fast Fourier Transform: betkaoui2010comparing; Image processing: qasaimeh2019comparing; Neural network: umuroglu2017finn
First, FPGAs have shown great energy efficiency because of their fully customizable circuits~\cite{qasaimeh2019comparing, betkaoui2010comparing, umuroglu2017finn}. 
Second, FPGAs are increasingly available in data centers and in the cloud~\cite{caulfield2016cloud, aqua}. %  MS, AWS, Alibaba, 
Third, FPGAs can be integrated with CPU on the same chip in the future according, making the reconfigurable hardware even more viable~\cite{kegel2020method}. %
As a result, big companies such as Microsoft, Amazon, Alibaba, and Baidu have adopted FPGAs for various workloads including machine learning inference, database acceleration, network offloading, and security operations~\cite{caulfield2016cloud, aqua, chen2022fidas, firestone2018azure}.
Due to the increasing popularity and the great potential of FPGAs, we study FPGA-based ANNS acceleration in this paper.

% For example, Microsoft catapult using big FPGA clusters for machine learning inference for Bing's web search. They also uses FPGAs for network-related workloads.
% Amazon put FPGAs close storage in their databases for query operator offloading. 
% Alibaba uses FPGAs for intrusion detection~\cite{}. % ISCA

% FPGA-based AI chips—such as Baidu’s Kunlun for AI, Alibaba’s Ouroboros for speech recognition, and Alibaba’s Hanguang 800 for inference operations—are deployed in their cloud data centers [43].
% Comparing Energy Efficiency of CPU, GPU and FPGA Implementations for Vision Kernels
% FPGAs show better energy efficiency compared to CPUs and GPUs in image processing
